Revisiting Few-sample BERT Fine-tuning

This paper is a study of fine-tuning of BERT contextual representations, with focus on commonly observed instabilities in few-sample scenarios. We identify several factors that cause this instability: the common use of a non-standard optimization method with biased gradient estimation; the limited applicability of significant parts of the BERT network for down-stream tasks; and the prevalent practice of using a pre-determined, and small number of training iterations. We empirically test the impact of these factors, and identify alternative practices that resolve the commonly observed instability of the process. In light of these observations, we re-visit recently proposed methods to improve few-sample fine-tuning with BERT and re-evaluate their effectiveness. Generally, we observe the impact of these methods diminishes significantly with our modified process.

==> data/dataset_stats.tex <==
\begin{tabular}{c|c|c|c}
    \toprule
    \multirow{2}{*}{Dataset} & \multicolumn{3}{c}{Number of examples} \\
    \cmidrule{2-4}
     & Train & Dev. & Test \\
    \midrule
    RTE & 2491 & 278 & 3001 \\
    MRPC & 3669 & 409 & 1726 \\
    STS-B & 5750 & 1380 & 1501 \\
    CoLA & 8551 & 1042 & 1064 \\
    MNLI* & 387703 & 5000 & 9816 \\
    QQP* & 358871 & 5000 & 40432 \\
    SST-2* & 62360 & 5000 & 873 \\
    CB & 250 & 56 & 249 \\
    BoolQ & 9427 & 3270 & 3244 \\
    UD-EWT & 12543 & 2002 & 2077 \\
    CoNLL-2003 & 14042 & 3254 & 3455 \\
    SQuAD* & 82599 & 5000 & 10570 \\
    \bottomrule
\end{tabular}

==> sections/impact.tex <==
\section*{Broader Impact}

Our work critically reviews and carefully investigates the current, broadly adopted optimization practices in \bert fine-tuning.
Our findings significantly stabilize \bert fine-tuning on small datasets. 
Stable training has multiple benefits. 
It reduces deployment costs and time,  potentially making  natural language processing applications more feasible and affordable for companies and individuals with limited computational resources. 
Our findings are focused on few-sample training scenarios, which opens, or at least eases the way for new applications at reduced data costs. 
The reduction in costs broadens the accessibility and reduces the energy footprint of \bert-based models. 
For example, applications that require frequent re-training are now easier to deploy given the reduced training costs.
Our work  also simplifies the scientific comparison between future fine-tuning methods by making training more stable, and therefore easier to reproduce. 
Our findings shed new light on several recently proposed techniques for \bert fine-tuning, potentially affecting methods relying on these techniques, which are not discussed in our paper.
More importantly, we recommend a set of solid optimization practices on which future research can be built upon.

Our work is applicable  to many different text processing applications. 
Societal impact largely depends on the application using our methods. We hope that broadening the set of organizations and individuals able to experiment with fine-tuning methods for a diverse set of tasks will allow for developing better informed  societal norms about NLP applications. 
Similar to existing work using the same set of datasets as ours, our work may also be influenced by biases in these datasets. We use multiple broadly-used datasets to limit our exposure for specific dataset bias. 
We focus on fine-tuning dynamics, and therefore the risk of damage through application failure is less relevant. At worst, failure of our proposed practices will lead to lower performance in end applications. We generally recommend developers to consider the implications of low performance in their systems. These are often scenario specific. 




